Hoare-style Specifications as Correctness Conditions for Non-linearizable Concurrent Objects

Designing scalable concurrent objects, which can be efficiently used on multicore processors, often requires one to abandon standard specification techniques, such as linearizability, in favor of more relaxed consistency requirements. However, the variety of alternative correctness conditions makes it difficult to choose which one to employ in a particular case, and to compose them when using objects whose behaviors are specified via different criteria. The lack of syntactic verification methods for most of these criteria poses challenges in their systematic adoption and application. In this paper, we argue for using Hoare-style program logics as an alternative and uniform approach for specification and compositional formal verification of safety properties for concurrent objects and their client programs. Through a series of case studies, we demonstrate how an existing program logic for concurrency can be employed off-the-shelf to capture important state and history invariants, allowing one to explicitly quantify over interference of environment threads and provide intuitive and expressive Hoare-style specifications for several non-linearizable concurrent objects that were previously specified only via dedicated correctness criteria. We illustrate the adequacy of our specifications by verifying a number of concurrent client scenarios, that make use of the previously specified concurrent objects, capturing the essence of such correctness conditions as concurrency-aware linearizability, quiescent, and quantitative quiescent consistency. All examples described in this paper are verified mechanically in Coq.

==> Makefile <==
all: paper.pdf

paper.pdf: paper.tex abstract.tex lstcoq.tex mathpartir.sty bibmacros.bib references.bib proceedings.bib sigplanconf.cls defs.tex Makefile intro1.tex discussion.tex counting.tex overview1.tex related.tex cal1.tex background1.tex counter.pdf chist.pdf qclients.tex conclusion.tex chist2.pdf queue.pdf evaluation.tex exchanger_outline.tex oopsla2016.sty authors.tex exchange_code.tex client_fig.tex exchange_proof.tex
	pdflatex paper
	bibtex paper -min-crossrefs=5
	pdflatex paper
	pdflatex paper

cover: cover.tex
	pdflatex cover
	pdflatex cover

# comments: paper.tex abstract.tex lstcoq.tex mathpartir.sty bibmacros.bib references.bib proceedings.bib sigplanconf.cls defs.tex Makefile intro1.tex discussion.tex counting.tex overview1.tex related.tex cal1.tex background.tex background1.tex counter.pdf chist.pdf qclients.tex conclusion.tex chist2.pdf queue.pdf evaluation.tex exchanger_outline.tex
# 	pdflatex --jobname=paper-commented "\def\extcomm{}\input{paper}"
# 	bibtex paper-commented -min-crossrefs=5
# 	pdflatex --jobname=paper-commented "\def\extcomm{}\input{paper}"
# 	pdflatex --jobname=paper-commented "\def\extcomm{}\input{paper}"

# ext: paper.tex abstract.tex lstcoq.tex mathpartir.sty bibmacros.bib references.bib proceedings.bib sigplanconf.cls defs.tex Makefile intro1.tex discussion.tex counting.tex overview1.tex related.tex cal1.tex background.tex background1.tex counter.pdf chist.pdf qclients.tex conclusion.tex chist2.pdf queue.pdf evaluation.tex exchanger_outline.tex
# 	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"
# 	bibtex paper-extended -min-crossrefs=5
# 	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"
# 	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"

quick:
	pdflatex paper




clean:
	rm -f *~ *.aux *.log *.blg *.dvi *.bm *.vrb *.toc *.nav *.out *.snm *.lof *.lot *.zip *.rel *.ps *.bbl paper.pdf
	rm -rf diff

zip:
	zip paper.zip paper.tex abstract.tex lstcoq.tex mathpartir.sty bibmacros.bib references.bib proceedings.bib sigplanconf.cls defs.tex Makefile intro1.tex discussion.tex counting.tex overview1.tex related.tex cal1.tex background.tex background1.tex counter.pdf chist.pdf qclients.tex conclusion.tex chist2.pdf queue.pdf evaluation.tex exchanger_outline.tex oopsla2016.sty paper.bbl authors.tex exchange_code.tex client_fig.tex exchange_proof.tex

prediff: paper.tex abstract.tex lstcoq.tex mathpartir.sty bibmacros.bib references.bib proceedings.bib sigplanconf.cls defs.tex Makefile intro1.tex discussion.tex counting.tex overview1.tex related.tex cal1.tex background1.tex counter.pdf chist.pdf qclients.tex conclusion.tex chist2.pdf queue.pdf evaluation.tex exchanger_outline.tex oopsla2016.sty authors.tex exchange_code.tex client_fig.tex exchange_proof.tex
	rm -rf diff
	mkdir diff
	cp ./{paper.tex,abstract.tex,authors.tex,exchange_code.tex,client_fig.tex,exchange_proof.tex,client_fig.tex,lstcoq.tex,mathpartir.sty,bibmacros.bib,references.bib,proceedings.bib,sigplanconf.cls,defs.tex,counter.pdf,chist.pdf,chist2.pdf,queue.pdf,oopsla2016.sty} diff
	latexdiff ../oopsla2016-first/paper.tex ./paper.tex > diff/paper.tex
	latexdiff ../oopsla2016-first/intro1.tex ./intro1.tex > diff/intro1.tex
	latexdiff ../oopsla2016-first/discussion.tex ./discussion.tex > diff/discussion.tex
	latexdiff ../oopsla2016-first/counting.tex ./counting.tex > diff/counting.tex
	latexdiff ../oopsla2016-first/overview1.tex ./overview1.tex > diff/overview1.tex
	latexdiff ../oopsla2016-first/cal1.tex ./cal1.tex > diff/cal1.tex
	latexdiff ../oopsla2016-first/background1.tex ./background1.tex > diff/background1.tex
	latexdiff ../oopsla2016-first/qclients.tex ./qclients.tex > diff/qclients.tex
	latexdiff ../oopsla2016-first/authors.tex ./authors.tex > diff/authors.tex
	latexdiff ../oopsla2016-first/conclusion.tex ./conclusion.tex > diff/conclusion.tex
	latexdiff ../oopsla2016-first/evaluation.tex ./evaluation.tex > diff/evaluation.tex
	latexdiff ../oopsla2016-first/related.tex ./related.tex > diff/related.tex
	latexdiff ../oopsla2016-first/exchanger_outline.tex ./exchanger_outline.tex > diff/exchanger_outline.tex


diff: prediff
	cd ./diff; pdflatex paper; bibtex paper -min-crossrefs=5; pdflatex paper; pdflatex paper


cleandiff:
	rm -rf diff

